Re-educating Educated Ones: A Case Study on Chakma Language Revitalization in Chittagong Hill Tracts

Indigenous languages face significant cultural oppression from official state languages, particularly in the Global South. We investigate the Bangladeshi Chakma language revitalization movement, a community grappling with language liquidity and amalgamation into the dominant Bengali language. Our six-month-long qualitative study involving interviews and focus group discussions with Chakma language learning stakeholders uncovered existing community socio-economic challenges and resilience strategies. We noted the need for culturally grounded digital tools and resources. We propose an ICT-mediated community-centric framework for Indigenous language revitalization in the Global South, emphasizing the integration of historical identity elements, stakeholder-defined requirements, and effective digital engagement strategies to empower communities in preserving their linguistic and cultural heritage.

==> Tables/codebook.tex <==
\section*{Codebook}
For our readers’ better understanding of our data analysis process, we provide examples of some themes/high-level codes and subthemes/codes along with their explanations/definitions below:

\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{6pt}

\begin{longtable}{|p{3cm}|p{8cm}|p{5cm}|}
\hline
\textbf{Themes/High Level Codes} & \textbf{Subtheme/Codes with Examples} & \textbf{Explanations/Definitions} \\
\hline
\endfirsthead

\hline
\textbf{Themes/High Level Codes} & \textbf{Subtheme/Codes with Examples} & \textbf{Explanations/Definitions} \\
\hline
\endhead

\multirow{3}{3cm}{\textbf{Design Implications and Challenges}} &
``Not everyone has a smartphone. Personally, I don’t have a smartphone either. What I use is a desktop,
which Basanti Di (Basanti Chakma, former MP) gave us for office use, and that’s what I use.'' -- Limited Access to ICTs &
Organizations reported limited technological support, with many instructors and learners lacking smartphones or computers and relying on traditional board-marker teaching. \\
\cline{2-3}
& `` We have members; we have 144 members from various upazilas. We ask them to in-quire at different schools, asking, ’We want to conduct a course on the Chakma language here, do you give us permission?’For works like these, a huge amount of money is required. But we don’t have that much money, so we carry them out with the passion and determination we have for this work'' -- Financial Struggle & Financial struggles limit Chakma Language Learning Center (CLLC) organizations’ capacity to expand preservation work. \\
\cline{2-3}
& ``Before, I did not know how to write using the script, which is why I didn’t. Now I can write, but my
smartphone doesn’t support the Chakma keyboard. It (OS) is an older version.'' -- Device and Font Limitations &
Devices often do not support Chakma fonts, preventing their use even when users can write the script. \\
\hline

\multirow{3}{3cm}{\textbf{Language, Sovereignty, and Imagined Communities}} &
``Our organization is almost one and a half years old, and we have organized 15–16 programs. In these
programs, we did not use Bangla fonts in the banner; rather, we used all Chakma fonts! It is up to
you if you can understand it or not! If the invited guests do not understand it, then we will translate
them.'' -- Enforcing Chakma Language in Oral and Written Communication &
Organizations pursue strong enforcement measures as part of revitalization, framing language not merely as a tool but as a marker of identity. \\
\cline{2-3}
& ``This is exactly what I’m talking about – technology is needed. The current generation reads less and
is averse to books. But if we could use technology properly, like creating cartoons, films, short films, or
even cartoons with Chakma rhymes, it could make a huge difference.'' -- Cultural Media Solutions &
Culturally grounded media (animations, rhymes, films) can capture youth attention and embed Chakma language into daily entertainment. \\
\cline{2-3}
& ``We created a Messenger group for those who participated. So, if we face any issues with spelling, we
ask questions there. Since several people participated in the workshop, there was always someone in
that group who knew the correct answer.'' -- Online Community Practices &
Online groups provide collaborative spaces for peer learning and knowledge exchange. \\
\hline

\multirow{3}{3cm}{\textbf{Methodological Framework: An ICT-Mediated, Community-Centric Approach}} &
``This is exactly what I’m talking about – technology is needed. The current generation reads less and
is averse to books. But if we could use technology properly, like creating cartoons, films, short films, or
even cartoons with Chakma rhymes, it could make a huge difference.'' - Cultural Media Solutions & Beyond functional tools, emphasize the importance of culturally
grounded media to revitalize interest in Chakma learning. 
 \\
\cline{2-3}
& ``“Well, right now, a lot of us are learning Korean, Chinese, Japanese, and also English, since it’s an
international language. So if we could build a translation app on Facebook, that would really help. Or,
let’s say we wanted to talk to foreigners—if we could translate our language into theirs, and theirs into
ours, it would make communication easier for them too'' -  Functional Digital Tools & Translation was viewed as a bridge between Chakma and dominant languages, encouraging expression a nd making
communication more inclusive
 \\
\cline{2-3}
& ``I think a mobile app could be really helpful. I would want it to tell me whether what I wrote is correct
or not. It should follow some standards, for instance, be accurate, like 80 or 90 percent at least. Not
online, an offline dictionary would be even more helpful.'' - Functional Digital Tools & The need for practical digital tools to support the
learning and everyday use of the Chakma script.
 \\
\hline

\end{longtable}
